Learning to Unlearn: Instance-wise Unlearning for Pre-trained Classifiers

Since the recent advent of regulations for data protection (e.g., the General Data Protection Regulation), there has been increasing demand in deleting information learned from sensitive data in pre-trained models without retraining from scratch. The inherent vulnerability of neural networks towards adversarial attacks and unfairness also calls for a robust method to remove or correct information in an instance-wise fashion, while retaining the predictive performance across remaining data. To this end, we consider instance-wise unlearning, of which the goal is to delete information on a set of instances from a pre-trained model, by either misclassifying each instance away from its original prediction or relabeling the instance to a different label. We also propose two methods that reduce forgetting on the remaining data: 1) utilizing adversarial examples to overcome forgetting at the representation-level and 2) leveraging weight importance metrics to pinpoint network parameters guilty of propagating unwanted information. Both methods only require the pre-trained model and data instances to forget, allowing painless application to real-life settings where the entire training set is unavailable. Through extensive experimentation on various image classification benchmarks, we show that our approach effectively preserves knowledge of remaining data while unlearning given instances in both single-task and continual unlearning scenarios.

==> Figures_tex/cifar100_various_model.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[MobileNetv2~\cite{(mobilenetv2)sandler2018mobilenetv2}]{
        \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures/cifar100_mobilenetv2_Dr.png}%
        \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures/cifar100_mobilenetv2_Df.png}%
        \includegraphics[height=3.35cm]{Figures/cifar100_mobilenetv2_Dtest.png}}
    \end{subfigure}
    
    \begin{subfigure}[SqueezeNet~\cite{(squeezenet)iandola2016squeezenet}]{
        \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures/squeezenet_MN_Dr.png}%
        \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/squeezenet_MN_Df.png}%
        \includegraphics[height=3.35cm]{Figures/squeezenet_MN_Dtest.png}}
    \end{subfigure}

    \begin{subfigure}[ViT~\cite{(vit)dosovitskiy2020image}]{
        \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/ViT_MN_Dr.png}%
        \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/ViT_MN_Dr.png}%
        \includegraphics[height=3.35cm]{Figures/ViT_MN_Dtest.png}}
    \end{subfigure}
    \caption{Experimental results before and after unlearning varying $k$ instances from various models on CIFAR-100.}
\label{fig:various_model_cifar100}
\end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[MobileNetv2~\cite{(mobilenetv2)sandler2018mobilenetv2}]{
%         \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures_2/mobilenetv2_MN_Dr (1).png}%
%         \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures_2/mobilenetv2_MN_Df (1).png}%
%         \includegraphics[height=3.35cm]{Figures_2/mobilenetv2_MN_Dtest (1).png}}
%     \end{subfigure}
    
%     \begin{subfigure}[SqueezeNet~\cite{(squeezenet)iandola2016squeezenet}]{
%         \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures_2/squeezenet_MN_Dr (1).png}%
%         \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures_2/squeezenet_MN_Df (1).png}%
%         \includegraphics[height=3.35cm]{Figures_2/squeezenet_MN_Dtest (1).png}}
%     \end{subfigure}

%     \begin{subfigure}[ViT~\cite{(vit)dosovitskiy2020image}]{
%         \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/ViT_MN_Dr.png}%
%         \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/ViT_MN_Dr.png}%
%         \includegraphics[height=3.35cm]{Figures/ViT_MN_Dtest.png}}
%     \end{subfigure}
%     \caption{Experimental results before and after unlearning varying $k$ instances from various models on CIFAR-100.}
% \label{fig:various_model_cifar100}
% \end{figure*}

==> Figures_tex/cka.tex <==
\begin{figure}[!t]
    %\vspace{-1mm}
    \centering
        \subfigure
        {\includegraphics[width=0.28\linewidth]{Figures/CKA_case1_Df.png}}
    %\vspace{-2mm}
        \subfigure
        {\includegraphics[width=0.28\linewidth]{Figures/CKA_case2_Df.png}}
    %\vspace{-2mm}
        \subfigure
        {\includegraphics[width=0.28\linewidth]{Figures/CKA_case3_Df.png}}
    %\vspace{-2mm}
        \addtocounter{subfigure}{-3} % needed for proper subfigure label
        \subfigure[\textsc{NegGrad}]
        {\includegraphics[width=0.28\linewidth]{Figures/CKA_case1_Dr.png}}
        \subfigure[\textsc{Adv}]
        {\includegraphics[width=0.28\linewidth]{Figures/CKA_case2_Dr.png}}
        \subfigure[\textsc{Adv+Imp}]
        {\includegraphics[width=0.28\linewidth]{Figures/CKA_case3_Dr.png}}
    
        % \begin{subfigure}[b]{.15\textwidth}
        %     \includegraphics[trim=17 17 54 22,clip,width=\textwidth]{Figures/CKA_case1_Df.png}
        % \end{subfigure}
        % \hfill
        % \begin{subfigure}[b]{.15\textwidth}
        %     \includegraphics[trim=17 17 54 22,clip,width=\textwidth]{Figures/CKA_case2_Df.png}
        % \end{subfigure}
        % \hfill
        % \begin{subfigure}[b]{.15\textwidth}
        %     \includegraphics[trim=17 17 54 22,clip,width=\textwidth]{Figures/CKA_case3_Df.png}
        % \end{subfigure}
        % \vfill
        % \begin{subfigure}[b]{.15\textwidth}
        %     \includegraphics[trim=17 17 54 22,clip,width=\textwidth]{Figures/CKA_case1_Dr.png}
        %     \vspace{-5mm}
        %     \caption{\textsc{NegGrad}}
        % \end{subfigure}
        % \hfill
        % \begin{subfigure}[b]{.15\textwidth}
        %     \includegraphics[trim=17 17 54 22,clip,width=\textwidth]{Figures/CKA_case2_Dr.png}
        %     \vspace{-5mm}
        %     \caption{\textsc{Adv}}
        % \end{subfigure}
        % \hfill
        % \begin{subfigure}[b]{.15\textwidth}
        %     \includegraphics[trim=17 17 54 22,clip,width=\textwidth]{Figures/CKA_case3_Dr.png}
        %     \vspace{-5mm}
        %     \caption{\textsc{Adv+Imp}}
        % \end{subfigure}
    %\vspace{-4mm}
    \caption{Layer-wise CKA correlations on $\mathcal{D}_f$ (top row) and $\mathcal{D}_r$ (bottom row) between representations before (X-axis) and after (Y-axis) unlearning. Brighter color indicates higher CKA correlation. \textsc{NegGrad} results in large forgetting of high-level features in both $\mathcal{D}_f$ and $\mathcal{D}_r$. Our approaches selectively forget high-level features only in $\mathcal{D}_f$.}
    \label{fig:cka}
    %\vspace{-0.5cm}
\end{figure}

==> Figures_tex/confusion_matrix.tex <==
% \begin{wrapfigure}{R}{.5\textwidth}
\begin{figure}[t!]
    % \vspace{-6.0mm}
    \centering
    %\hspace{-6.0mm}
        \subfigure[\textsc{NegGrad}]
        {\includegraphics[width=0.35\linewidth]{Figures/after_neggrad_true.png}}
    \hspace{-6.0mm}
        \subfigure[\textsc{Adv}]
        {\includegraphics[width=0.35\linewidth]{Figures/after_adv.png}}
    \hspace{-6.0mm}
        \subfigure[\textsc{Adv+Imp}]
        {\includegraphics[width=0.35\linewidth]{Figures/after_adv_imp.png}}
    %\hspace{-6.0mm}
        % \begin{subfigure}{0.2\textwidth}
        %     \includegraphics[trim=40 20 115 40,clip,width=0.05\textwidth]{Figures/after_neggrad_true.png}
        %     \caption{\textsc{NegGrad}}
        % \end{subfigure}
        % \hfill
        % \begin{subfigure}{0.2\textwidth}
        %     \includegraphics[trim=40 20 115 40,clip,width=0.05\textwidth]{Figures/after_adv.png}
        %     \caption{\textsc{Adv}}
        % \end{subfigure}
        % \hfill
        % \begin{subfigure}{0.2\textwidth}
        %     \includegraphics[trim=40 20 115 40,clip,width=0.05\textwidth]{Figures/after_adv_imp.png}
        %     \caption{\textsc{Adv+Imp}}
        % \end{subfigure}
    %\vspace{-5mm}
    \caption{Confusion matrices showing average pairwise frequencies of pre- (Y-axis) and post-unlearning (X-axis) prediction labels from $\mathcal{D}_f$. A blue color indicates higher frequency. Our unlearning framework does not produce any discernible correlation in misclassification.}
%\vspace{-0.5cm}
    \label{fig:confusion_matrix}
\end{figure}
% \end{wrapfigure}


% \begin{figure}
% \begin{subfigure}[h]{0.4\columnwidth}
%     \includegraphics[width=\linewidth]{Figures/after_neggrad_true.png}
%     \caption{Picture 1}
%     \label{fig:1}
%   \end{subfigure}
%   \hfill %%
%   \begin{subfigure}[h]{0.4\columnwidth}
%     \includegraphics[width=\linewidth]{Figures/after_neggrad_true.png}
%     \caption{Picture 2}
%     \label{fig:2}
%   \end{subfigure}
% \end{figure}

==> Figures_tex/decision_boundary.tex <==
% \vspace{-0.5cm}
\begin{figure*}[!h]
    %\vspace{-0.3cm}
    \centering
    \subfigure[\textsc{Before}]
    {\includegraphics[width=0.2\linewidth]{Figures/decision_boundary_before.png}}
    \subfigure[\textsc{NegGrad}]
    {\includegraphics[width=0.2\linewidth]{Figures/decision_boundary_case1.png}}
    \subfigure[\textsc{Adv}]
    {\includegraphics[width=0.2\linewidth]{Figures/decision_boundary_case2.png}}
    \subfigure[\textsc{Adv+Imp}]
    {\includegraphics[width=0.2\linewidth]{Figures/decision_boundary_case3.png}}
    % \begin{subfigure}[b]{.23\textwidth}
    %     \includegraphics[width=\textwidth]{Figures/decision_boundary_before.png}
    %     \vspace{-5mm}
    %     \caption{\textsc{Before}}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{.23\textwidth}
    %     \includegraphics[width=\textwidth]{Figures/decision_boundary_case1.png}
    %     \vspace{-5mm}
    %     \caption{\textsc{NegGrad}}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{.23\textwidth}
    %     \includegraphics[width=\textwidth]{Figures/decision_boundary_case2.png}
    %     \vspace{-5mm}
    %     \caption{\textsc{Adv}}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{.23\textwidth}
    %     \includegraphics[width=\textwidth]{Figures/decision_boundary_case3.png}
    %     \vspace{-5mm}
    %     \caption{\textsc{Adv+Imp}}
    % \end{subfigure}
    %\vspace{-3mm}
    \caption{t-SNE plots of CIFAR-10 datapoints in $\mathcal{D}_f$ (triangles) and $\mathcal{D}_r$ (dots) before and after unlearning. Colors indicate true labels for all plots. Regularization with adversarial examples and weight importance effectively preserves the decision boundary while migrating instances in $\mathcal{D}_f$ towards the class boundary to induce misclassification.}
    %\vspace{-5mm}
    \label{fig:decision_boundary}
\end{figure*}
% % HL: Visualization 상으로는 특정 class의 representation/decision boundary가 많이 바뀌는 것 같은데 괜찮은 것인가요? 특히 tSNE plot 왼쪽 부분의 purple, magenta cluster 상대적 위치가 바뀌는 걸로 보입니다.
% % SJ: 말씀대로 decision boundary의 변화도 있고, 각 instance마다 가까운 다른 cluster로 가지는 않는다는 visualization이 이전에 나왔었는데, 이는 high-dimensional feature space라는 점과 tSNE plot자체의 stochasticity에서 나오는것으로 보고 있습니다. 여기서 보여주고자 했던점은 class-level에서의 구분 능력은 유지가 된다는것이라 이것을 중점적으로 서술을 해야할것같습니다.


==> Figures_tex/decision_boundary_2rows.tex <==
% \vspace{-0.5cm}
\begin{figure}[!h]
    %\vspace{-0.3cm}
    \centering
    \subfigure[\textsc{Before}]
    {\includegraphics[width=0.45\linewidth]{Figures/decision_boundary_before.png}}
    \vspace{-3mm}
    \subfigure[\textsc{NegGrad}]
    {\includegraphics[width=0.45\linewidth]{Figures/decision_boundary_case1.png}}
    \vspace{-3mm}
    \subfigure[\textsc{Adv}]
    {\includegraphics[width=0.45\linewidth]{Figures/decision_boundary_case2.png}}
    \subfigure[\textsc{Adv+Imp}]
    {\includegraphics[width=0.45\linewidth]{Figures/decision_boundary_case3.png}}
    \caption{t-SNE plots of CIFAR-10 datapoints in $\mathcal{D}_f$ (triangles) and $\mathcal{D}_r$ (dots) before and after unlearning. Colors indicate true labels for all plots. Regularization with adversarial examples and weight importance effectively preserves the decision boundary while migrating instances in $\mathcal{D}_f$ towards the class boundary to induce misclassification.}
    \vspace{-5mm}
    \label{fig:decision_boundary}
\end{figure}
% % HL: Visualization 상으로는 특정 class의 representation/decision boundary가 많이 바뀌는 것 같은데 괜찮은 것인가요? 특히 tSNE plot 왼쪽 부분의 purple, magenta cluster 상대적 위치가 바뀌는 걸로 보입니다.
% % SJ: 말씀대로 decision boundary의 변화도 있고, 각 instance마다 가까운 다른 cluster로 가지는 않는다는 visualization이 이전에 나왔었는데, 이는 high-dimensional feature space라는 점과 tSNE plot자체의 stochasticity에서 나오는것으로 보고 있습니다. 여기서 보여주고자 했던점은 class-level에서의 구분 능력은 유지가 된다는것이라 이것을 중점적으로 서술을 해야할것같습니다.


==> Figures_tex/imagenet_various_model.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[MobileNet v2~\cite{(mobilenetv2)sandler2018mobilenetv2}]{
        \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures/mobilenet_img_Dr.png}%
        \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/mobilenet_img_Df.png}%
        \includegraphics[height=3.35cm]{Figures/mobilenet_img_Dtest.png}}
        % \caption{MobileNet v2}
    \end{subfigure}
    \begin{subfigure}[ResNet34~\cite{(resnet)he2016deep}]{
        \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/resnet34_img_Dr.png}%
        \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/resnet34_img_Df.png}%
        \includegraphics[height=3.35cm]{Figures/resnet34_img_Dtest.png}}
        % \caption{ResNet34}
    \end{subfigure}
    \begin{subfigure}[DenseNet121~\cite{(densenet)huang2017densely}]{
        \includegraphics[trim=0 0 80 0,clip,height=3.35cm]{Figures/densenet121_img_Dr.png}%
        \includegraphics[trim=0 0 80 0, clip,height=3.35cm]{Figures/densenet121_img_Df.png}%
        \includegraphics[height=3.35cm]{Figures/densenet121_img_Dtest.png}}
        % \caption{DenseNet121}
    \end{subfigure}
    \caption{Experimental results before and after unlearning varying $k$ instances from various models on ImageNet-1K.}
    \label{fig:various_model_imagenet}
\end{figure*}

==> Tables_tex/cifar100_various_model.tex <==
\begin{table*}[!t]
\caption{Evaluation results before and after unlearning $k$ instances from various pretrained models. Our approach is model-agnostic and is effective in preserving knowledge of $\mathcal{D}_r$ across different architectures.}
\vspace{-.1in}  
\centering
\smallskip\noindent
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|cccc|cccc|cccc}
\toprule
&  & \multicolumn{4}{c|}{SqueezeNet~\citep{(squeezenet)iandola2016squeezenet}} & \multicolumn{4}{c|}{MobileNetv2~\citep{(mobilenetv2)sandler2018mobilenetv2}} & \multicolumn{4}{c}{ViT~\citep{(vit)dosovitskiy2020image}}\\ 
&  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  \\ \midrule
\multirow{4}{*}{$D_f$ ($\downarrow$)} 
& Before & 91.67 & 93.75 & 95.83 & 96.61 & 100.0 & 89.58 & 88.54 & 92.45 & 100.0 & 100.0 & 100.0 & 100.0\\
& NegGrad  & 0.0  & 0.0 & 0.0 & 0.0 & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.26 \\
& Adv  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  & 0.0 & 0.0 & 0.0 & 8.33 & 0.0 & 0.0 & 0.0  \\
& Adv+Imp  & 0.0 & 0.0 & 0.0 & 1.82 &  0.0 & 0.0 & 0.0 & 3.13 & 16.67 & 16.67 & 2.61 & 3.52 \\
\midrule
\multirow{4}{*}{$D_r$ ($\uparrow$)}   
& Before & 96.26 & 96.26 & 96.26 & 96.26 & 91.73 & 91.73 & 91.74 & 91.73 & 99.70 & 99.70 & 99.70 & 99.70\\
& NegGrad & \textbf{69.97} & 46.84 & 29.29 & 20.51 &\textbf{79.60} & 50.69 & 25.83 & 18.91 & 57.28 & 1.85 & 1.65 & 1.01 \\
& Adv & 53.38 & \textbf{64.82} & 60.99 & 54.16 & 49.35 & 57.09 & 47.57 & 41.68 & 87.39 & 43.46 & 10.96 & \textbf{5.58} \\
& Adv+Imp & 52.97 & 64.72 & \textbf{66.37} & \textbf{60.04} & 49.27 & \textbf{58.20} & \textbf{55.09} & \textbf{48.60} & \textbf{87.41} & \textbf{58.63} & \textbf{13.73} & 5.02 \\ 
\midrule
\multirow{4}{*}{$D_{test}$ ($\uparrow$)} 
& Before & 69.19 & 69.19 & 69.19 & 69.19 & 67.11 & 67.11 & 67.11 & 67.11 & 89.85 & 89.85 & 89.85 & 89.85 \\
& NegGrad & 52.63 & 37.33 & 23.50 & 16.46 & \textbf{60.11} & 41.38 & 22.55 & 16.24 & 49.62 & 1.73 & 1.71 & 1.01 \\
& Adv & \textbf{42.55} & 49.18 & 45.43 & 40.10 & 41.18 & 46.99 & 39.43 & 34.60 & \textbf{73.83} & 36.04 & 9.24 & \textbf{4.79} \\
& Adv+Imp & 42.16 & \textbf{49.24} & \textbf{48.96} & \textbf{44.01} & 41.15 & \textbf{47.58} & \textbf{44.89} & \textbf{39.54} & 73.33 & \textbf{48.18} & \textbf{11.64} & 4.43 \\
\bottomrule
\end{tabular}
}
% \vspace{-.25in}
\label{table:main_result_models}
\end{table*}



% \begin{table*}[!tp]
% \caption{Evaluation results before and after unlearning $k$ instances from pretrained checkpoints of various model architectures. Our approach is model-agnostic and is effective in preserving knowledge of $\mathcal{D}_r$ across different architectures.}
% \vspace{-.1in}  
% \centering
% \smallskip\noindent
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ll|cccc|cccc|cccc}
% \toprule
% &  & \multicolumn{4}{c|}{ResNet-34~\citep{(resnet)he2016deep}} & \multicolumn{4}{c|}{SqueezeNet~\citep{(squeezenet)iandola2016squeezenet}} & \multicolumn{4}{c}{ResNext-50~\citep{(resnext)xie2017aggregated}}\\ 
% &  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  \\ \midrule
% \multirow{4}{*}{$D_f$ ($\downarrow$)} 
% & Before &  100.0 & 100.0 & 100.0 & 100.0 & 91.67 & 93.75 & 95.83 & 96.61 & 100.0 & 100.0 & 100.0 &  100.0\\
% & NegGrad  & 0.0  & 0.0 & 0.0 & 0.0 & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% & Adv  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\
% & Adv+Imp  & 0.0 & 0.0 & 0.0 & 4.43 &  0.0 & 0.0 & 0.0 & 1.82 & 0.0 & 0.0 & 14.06 & 2.86 \\
% \midrule
% \multirow{4}{*}{$D_r$ ($\uparrow$)}   
% & Before & 99.97 & 99.97 & 99.97 & 99.97 &  96.26 & 96.26 & 96.26& 96.26 & 99.98 & 99.98 & 99.98 & 99.98 \\
% & NegGrad & \textbf{98.37} & 86.75 & 74.65 & 65.76 & \textbf{69.97} & 46.84 & 29.29 & 20.51 & \textbf{97.44} & 77.80 & 65.56 & 45.17   \\
% & Adv & 75.44 & \textbf{89.69} & \textbf{93.66} &\textbf{91.57} & 53.38 & \textbf{64.82} & 60.99 & 54.16 & 62.54 & \textbf{84.56} & 86.67 & \textbf{81.13}  \\
% & Adv+Imp & 75.41 & 88.17 & 83.14 & 80.32 & 52.97 & 64.72 & \textbf{66.37} & \textbf{60.04} & 62.45 & 83.65 & \textbf{88.34} & 55.34  \\ 
% \midrule
% \multirow{4}{*}{$D_{test}$ ($\uparrow$)} 
% & Before & 77.54 & 77.54 & 77.54 & 77.54 & 69.19 & 69.19 & 69.19 & 69.19 & 78.34 & 78.34 & 78.34 & 78.34  \\
% & NegGrad & \textbf{71.86} & 62.31 & 53.03 & 46.13 & 52.63 & 37.33 & 23.50 & 16.46 & \textbf{72.02} & 57.20 & 48.76 & 34.04 \\
% & Adv & 54.10 & \textbf{64.37} & \textbf{67.17} & \textbf{64.68} & \textbf{42.55} & 49.18 & 45.43 & 40.10 & 47.56 & \textbf{61.85} & 63.13 & \textbf{58.02} \\
% & Adv+Imp & 54.09 & 63.34 & 58.84 & 57.66 & 42.16 & \textbf{49.24} & \textbf{48.96} & \textbf{44.01} & 47.54 & 61.30 & \textbf{64.33} & 40.95 \\
% \midrule\midrule

% &  & \multicolumn{4}{c|}{DenseNet-121~\citep{(densenet)huang2017densely}} & \multicolumn{4}{c|}{MobileNetv2~\citep{(mobilenetv2)sandler2018mobilenetv2}} & \multicolumn{4}{c}{ViT~\citep{(vit)dosovitskiy2020image}}\\ 
% &  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  & {$k=4$} & {$k=16$} & {$k=64$}   & $k=128$  \\ \midrule
% \multirow{4}{*}{$D_f$ ($\downarrow$)} 
% & Before & 100.0 & 100.0 & 100.0 &  100.0  & 100.0 & 89.58 & 88.54 & 92.45 & 100.0 & 100.0 & 100.0 & 100.0 \\
% & NegGrad & 0.0  & 0.0 & 0.0 & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.26 \\
% & Adv & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 8.33 & 0.0 & 0.0 & 0.0 \\
% & Adv+Imp  & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 3.13 & 16.67 & 16.67 & 2.61 & 3.52 \\
% \midrule
% \multirow{4}{*}{$D_r$ ($\uparrow$)}   
% & Before & 99.98 & 99.98 & 99.98 & 99.98 & 91.73 & 91.73 & 91.74 & 91.73 & 99.70 & 99.70 & 99.70 & 99.70 \\
% & NegGrad & \textbf{98.24} & 77.97 & 63.19 & 52.23 & \textbf{79.60} & 50.69 & 25.83 & 18.91 & 57.28 & 1.85 & 1.65 & 1.01 \\
% & Adv & 69.34 & \textbf{85.90} & \textbf{89.88} & \textbf{83.03} &  49.35 & 57.09 & 47.57 & 41.68 & 87.39 & 43.46 & 10.96 & \textbf{5.58} \\
% & Adv+Imp & 69.26 & 85.67 & 84.01 & 16.27 & 49.27 & \textbf{58.20} & \textbf{55.09} & \textbf{48.60} & \textbf{87.41} & \textbf{58.63} & \textbf{13.73} & 5.02 \\ 
% \midrule
% \multirow{4}{*}{$D_{test}$ ($\uparrow$)} 
% & Before & 79.11 & 79.11 & 79.11 &  79.11 & 67.11 & 67.11 & 67.11 & 67.11 & 89.85 & 89.85 & 89.85 & 89.85 \\
% & NegGrad & \textbf{73.45} & 57.26 & 46.19 & 38.69 & \textbf{60.11} & 41.38 & 22.55 & 16.24 & 49.62 & 1.73 & 1.71 & 1.01 \\
% & Adv & 51.40  & \textbf{62.86} & \textbf{64.91} & \textbf{58.12} & 41.18 & 46.99 & 39.43 & 34.6 & \textbf{73.83} & 36.04 & 9.24 & \textbf{4.79} \\
% & Adv+Imp & 51.36 & 62.50 & 60.14 & 12.35 & 41.15 & \textbf{47.58} & \textbf{44.89} & \textbf{39.54} & 73.33 & \textbf{48.18} & \textbf{11.64} & 4.43 \\
% \bottomrule
% \end{tabular}
% }
% % \vspace{-.25in}
% \label{table:main_result_models}
% \end{table*}


==> Tables_tex/imagenet_various_model.tex <==
\begin{table*}[!tp]
\caption{Evaluation results before and after unlearning $k$ instances from pretrained checkpoints of various model architectures. Our approach is model-agnostic and is effective in preserving knowledge of $\mathcal{D}_r$ across different architectures.}
\vspace{-.1in}  
\centering
\smallskip\noindent
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|cccc|cccc|cccc}
\toprule
&  & \multicolumn{4}{c|}{ResNet-34~\citep{(resnet)he2016deep}} & \multicolumn{4}{c|}{SqueezeNet~\citep{(squeezenet)iandola2016squeezenet}} & \multicolumn{4}{c}{ResNext-50~\citep{(resnext)xie2017aggregated}}\\ 
&  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  \\ \midrule
\multirow{4}{*}{$D_f$ ($\downarrow$)} 
& Before &  100.0 & 100.0 & 100.0 & 100.0 & 91.67 & 93.75 & 95.83 & 96.61 & 100.0 & 100.0 & 100.0 &  100.0\\
& NegGrad  & 0.0  & 0.0 & 0.0 & 0.0 & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
& Adv  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\
& Adv+Imp  & 0.0 & 0.0 & 0.0 & 4.43 &  0.0 & 0.0 & 0.0 & 1.82 & 0.0 & 0.0 & 14.06 & 2.86 \\
\midrule
\multirow{4}{*}{$D_r$ ($\uparrow$)}   
& Before & 99.97 & 99.97 & 99.97 & 99.97 &  96.26 & 96.26 & 96.26& 96.26 & 99.98 & 99.98 & 99.98 & 99.98 \\
& NegGrad & \textbf{98.37} & 86.75 & 74.65 & 65.76 & \textbf{69.97} & 46.84 & 29.29 & 20.51 & \textbf{97.44} & 77.80 & 65.56 & 45.17   \\
& Adv & 75.44 & \textbf{89.69} & \textbf{93.66} &\textbf{91.57} & 53.38 & \textbf{64.82} & 60.99 & 54.16 & 62.54 & \textbf{84.56} & 86.67 & \textbf{81.13}  \\
& Adv+Imp & 75.41 & 88.17 & 83.14 & 80.32 & 52.97 & 64.72 & \textbf{66.37} & \textbf{60.04} & 62.45 & 83.65 & \textbf{88.34} & 55.34  \\ 
\midrule
\multirow{4}{*}{$D_{test}$ ($\uparrow$)} 
& Before & 77.54 & 77.54 & 77.54 & 77.54 & 69.19 & 69.19 & 69.19 & 69.19 & 78.34 & 78.34 & 78.34 & 78.34  \\
& NegGrad & \textbf{71.86} & 62.31 & 53.03 & 46.13 & 52.63 & 37.33 & 23.50 & 16.46 & \textbf{72.02} & 57.20 & 48.76 & 34.04 \\
& Adv & 54.10 & \textbf{64.37} & \textbf{67.17} & \textbf{64.68} & \textbf{42.55} & 49.18 & 45.43 & 40.10 & 47.56 & \textbf{61.85} & 63.13 & \textbf{58.02} \\
& Adv+Imp & 54.09 & 63.34 & 58.84 & 57.66 & 42.16 & \textbf{49.24} & \textbf{48.96} & \textbf{44.01} & 47.54 & 61.30 & \textbf{64.33} & 40.95 \\
\midrule\midrule

&  & \multicolumn{4}{c|}{DenseNet-121~\citep{(densenet)huang2017densely}} & \multicolumn{4}{c|}{MobileNetv2~\citep{(mobilenetv2)sandler2018mobilenetv2}} & \multicolumn{4}{c}{ViT~\citep{(vit)dosovitskiy2020image}}\\ 
&  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  & {$k=4$} & {$k=16$} & {$k=64$}   & $k=128$  \\ \midrule
\multirow{4}{*}{$D_f$ ($\downarrow$)} 
& Before & 100.0 & 100.0 & 100.0 &  100.0  &  &  &  &  &  &  &  &  \\
& NegGrad & 0.0  & 0.0 & 0.0 & 0.0  &  &  &  &  &  &  &  &  \\
& Adv & 0.0  & 0.0 & 0.0 & 0.0&  &  &  &  &  &  &  &  \\
& Adv+Imp  & 0.0  & 0.0 & 0.0 & 0.0 &  &  &  &  &  &  &  &  \\
\midrule
\multirow{4}{*}{$D_r$ ($\uparrow$)}   
& Before & 99.98 & 99.98 & 99.98 & 99.98 &  &  &  &  &  &  &  &  \\
& NegGrad & \textbf{98.24} & 77.97 & 63.19 & 52.23 &  &  &  &  &  &  &  &  \\
& Adv & 69.34 & \textbf{85.90} & \textbf{89.88} & \textbf{83.03 }&  &  &  &  &  &  &  &  \\
& Adv+Imp & 69.26 & 85.67 & 84.01 & 16.27 &  &  &  &  &  &  &  &  \\ 
\midrule
\multirow{4}{*}{$D_{test}$ ($\uparrow$)} 
& Before & 79.11 & 79.11 & 79.11 &  79.11 &  &  &  &  &  &  &  &  \\
& NegGrad & \textbf{73.45} & 57.26 & 46.19 & 38.69 &  &  &  &  &  &  &  &  \\
& Adv & 51.40  & \textbf{62.86} & \textbf{64.91} & \textbf{58.12} &  &  &  &  &  &  &  &  \\
& Adv+Imp & 51.36 & 62.50 & 60.14 & 12.35 &  &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
% \vspace{-.25in}
\label{table:main_result_models}
\end{table*}


==> Tables_tex/main_table.tex <==
\begin{table*}[!tp]
\footnotesize
\caption{Evaluation results before and after unlearning $k$ instances \csm{from ResNet-18 (for CIFAR-10) and ResNet-50 (for CIFAR-100 and ImageNet-1K)} pretrained on respective image classification datasets. While using negative gradients only loses significant information on $\mathcal{D}_r$, our proposed methods \textsc{Adv} and \textsc{Adv+Imp} retain predictive performance on $\mathcal{D}_r$ as well as $\mathcal{D}_{test}$, while completely forgetting instances in $\mathcal{D}_f$.}
%\vspace{-.1in}  
\centering
\smallskip\noindent
\resizebox{.9\linewidth}{!}{
\begin{tabular}{ll|cccc|cccc|cccc}
\toprule
&  & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{CIFAR-100} & \multicolumn{4}{c}{ImageNet-1K}\\ 
&  & {$k=16$} & {$k=64$} & $k=128$ & $k=256$  & {$k=16$} & {$k=64$} & $k=128$ & $k=256$    & {$k=16$} & {$k=64$} & $k=128$ & $k=256$   \\ \midrule
\multirow{5}{*}{$D_f$ ($\downarrow$)} 
& \textsc{Before} & {100.0} & {99.38} & 99.53 & 99.38 & {100.0} & {100.0} & 100.0 & 100.0 & {87.50} & {84.69} & 86.09 & 86.02 \\
& \textsc{Oracle}  &  0.0 &  0.0 &  0.0 & 0.63 &  0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0  & 0.26  & 5.73   \\ 
& \textsc{NegGrad}  & 0.0   & 0.0   & 0.0   & 3.83   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   \\ 
& \textsc{RAWP} & 0.0   & 0.0   & 4.06   & 6.17   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    \\ 
& \textsc{Adv}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   \\ 
& \textsc{Adv+Imp}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 2.73\\ 
\midrule
\multirow{5}{*}{$D_r$ ($\uparrow$)}    
& \textsc{Before} & {99.60} & {99.60} & 99.60 & 99.60 & {99.98} & {99.98} & 99.98 & 99.98 & {87.42} & {87.42} & 87.42 & 87.42\\
& \textsc{Oracle}  & 98.74  & 99.72  & 98.97 & 39.90 & 99.96 & 96.17  & 96.74 & 96.43 &  73.36 & 77.81 & 67.7 &  61.61 \\
& \textsc{NegGrad}  & {15.79} & {9.22}  & 7.11  & 6.34 & {66.97} & {26.20} & 11.64 & 1.70 & {65.02} & {35.66} & 19.27 & 0.48\\
& \textsc{RAWP}  & 67.15  & 37.32 & 13.28 & 9.12 & 72.44  & 17.39 & 2.82 & 1.12   & 20.33 & 2.72 & 0.29 & 0.10  \\ 
& \textsc{Adv}  & {69.70} & {66.97} & 53.49 & 39.33 & {89.18} & {81.07} & 76.28 & 65.67 & {80.92} & {73.60} & 66.31 & 43.70\\
& \textsc{Adv+Imp}  & {\textbf{85.75}} & {\textbf{72.77}} & \textbf{54.51} & \textbf{48.95} & {\textbf{89.91}} & {\textbf{89.48}} & \textbf{82.86} & \textbf{67.60} & {\textbf{81.43}} & {\textbf{79.03}} & \textbf{74.14} & \textbf{65.32}\\ 
\midrule
\multirow{5}{*}{$D_{test}$ ($\uparrow$)} 
& \textsc{Before} & {92.59} & {92.59} & 92.59 & 92.59 & {77.10} & {77.10} & 77.10 & 77.10  & {76.01} & {76.01} & 76.01 & 76.01\\
& \textsc{Oracle}  & 90.21 &  91.01 &  89.44 & 38.59 & 64.41 & 67.06 & 66.88 & 65.31 & 63.91 & 68.08 & 59.09 &  54.03 \\ 
& \textsc{NegGrad} & {15.87} & {9.28}  & 7.11  & 6.47 & {48.07} & {21.11} & 10.19 &  1.71 & {56.70} & {31.10} & 17.08 & 0.46\\
& \textsc{RAWP}  & 63.10 & 35.47 & 12.91 & 9.12 & 50.99 & 14.41  & 2.79 & 1.12 & 17.53 & 2.41 & 0.28 & 0.10  \\ 
& \textsc{Adv}  & {65.14} & {62.23} & 49.47 & 36.69 & {63.17} & {57.43} & 53.89 & 46.45 & {70.36} & {65.51} & 57.34 & 38.25\\
& \textsc{Adv+Imp}  & {\textbf{79.65}} & {\textbf{67.08}} & \textbf{50.82} & \textbf{45.44} & {\textbf{63.69}} & {\textbf{62.83}} & \textbf{58.44} & \textbf{48.71} & {\textbf{70.77}} & {\textbf{68.43}} & \textbf{64.05} & \textbf{56.52}\\ 
\bottomrule
\end{tabular}}
\label{table:main_result_dataset}
%\vspace{-3mm}
\end{table*}

% \begin{table*}[!tp]
% \caption{Evaluation results before and after unlearning $k$ instances from ResNet-50 pretrained on respective image classification datasets. While using negative gradients only loses significant information on $\mathcal{D}_r$, our proposed methods \textsc{Adv} and \textsc{Adv+Imp} retain predictive performance on $\mathcal{D}_r$ as well as $\mathcal{D}_{test}$, while completely forgetting instances in $\mathcal{D}_f$.}
% \vspace{-.1in}  
% \centering
% \smallskip\noindent
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ll|cccc|cccc}
% \toprule
% &  & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{CIFAR-100} \\ 
% &  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$ \\ \midrule
% \multirow{4}{*}{$D_f$ ($\downarrow$)} 
% & \textsc{Before} & {100.0} & {100.0} & {99.38} & 99.53 & {100.0} & {100.0} & {100.0} & 100.0 \\
% & \ds{\textsc{Oracle}}  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\ 
% & \textsc{NegGrad}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    \\ 
% & \textsc{Adv}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    \\ 
% & \textsc{Adv+Imp}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0 \\ 
% \midrule
% \multirow{5}{*}{$D_r$ ($\uparrow$)}   
% & \textsc{Before} & {99.60} & {99.60} & {99.60} & 99.60 & {99.98} & {99.98} & {99.98} & 99.9 \\
% & \ds{\textsc{Oracle}}  & 93.43 & 98.74 & 99.72 & 98.97 & 99.68 & 99.96 & 96.17 & 96.74\\ 
% & \textsc{NegGrad}  & {38.44} & {15.79} & {9.22}  & 7.11  & {\textbf{99.71}} & {66.97} & {26.20} & 11.64 \\
% & \textsc{Adv}  & {79.40} & {69.70} & {66.97} & 53.49 & {83.90} & {89.18} & {81.07} & 76.28  \\
% & \textsc{Adv+Imp}  & {\textbf{82.95}} & {\textbf{85.75}} & {\textbf{72.77}} & \textbf{54.51} & {83.89} & {\textbf{89.91}} & {\textbf{89.48}} & \textbf{82.86}\\ 
% \midrule
% \multirow{5}{*}{$D_{test}$ ($\uparrow$)} 
% & \textsc{Before} & {92.59} & {92.59} & {92.59} & 92.59 & {77.10} & {77.10} & {77.10} & 77.10  \\
% & \ds{\textsc{Oracle}} & 86.28 & 90.21 & 91.01 & 89.44 & 77.49 & 64.41 & 67.06 & 66.88\\ 
% & \textsc{NegGrad}  & {36.56} & {15.87} & {9.28}  & 7.11  & {\textbf{74.54}} & {48.07} & {21.11} & 10.19 \\
% & \textsc{Adv}  & {74.34} & {65.14} & {62.23} & 49.47 & {60.00}  & {63.17} & {57.43} & 53.89  \\
% & \textsc{Adv+Imp}  & {\textbf{77.53}} & {\textbf{79.65}} & {\textbf{67.08}} & \textbf{50.82} & {60.50} & {\textbf{63.69}} & {\textbf{62.83}} & \textbf{58.44} \\ 
% \bottomrule
% \end{tabular}}
% \vspace{-4mm}
% \label{table:main_result_dataset}
% \end{table*}


==> Tables_tex/oracle.tex <==

\begin{table*}[!tp]
\caption{Evaluation results before and after unlearning $k$ instances from ResNet-50 pretrained on respective image classification datasets. While using negative gradients only loses significant information on $\mathcal{D}_r$, our proposed methods \textsc{Adv} and \textsc{Adv+Imp} retain predictive performance on $\mathcal{D}_r$ as well as $\mathcal{D}_{test}$, while completely forgetting instances in $\mathcal{D}_f$.}
\vspace{-.1in}  
\centering
\smallskip\noindent
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|cccc|cccc}
\toprule
&  & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{CIFAR-100} \\ 
&  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$ \\ \midrule
\multirow{4}{*}{$D_f$ ($\downarrow$)} 
& \textsc{Before} & {100.0} & {100.0} & {99.38} & 99.53 & {100.0} & {100.0} & {100.0} & 100.0 \\
& \ds{\textsc{Oracle}}  & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\ 
& \textsc{NegGrad}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    \\ 
& \textsc{Adv}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    \\ 
& \textsc{Adv+Imp}  & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0 \\ 
\midrule
\multirow{5}{*}{$D_r$ ($\uparrow$)}   
& \textsc{Before} & {99.60} & {99.60} & {99.60} & 99.60 & {99.98} & {99.98} & {99.98} & 99.9 \\
& \ds{\textsc{Oracle}}  & 93.43 & 98.74 & 99.72 & 98.97 & 99.68 & 99.96 & 96.17 & 96.74\\ 
& \textsc{NegGrad}  & {38.44} & {15.79} & {9.22}  & 7.11  & {\textbf{99.71}} & {66.97} & {26.20} & 11.64 \\
& \textsc{Adv}  & {79.40} & {69.70} & {66.97} & 53.49 & {83.90} & {89.18} & {81.07} & 76.28  \\
& \textsc{Adv+Imp}  & {\textbf{82.95}} & {\textbf{85.75}} & {\textbf{72.77}} & \textbf{54.51} & {83.89} & {\textbf{89.91}} & {\textbf{89.48}} & \textbf{82.86}\\ 
\midrule
\multirow{5}{*}{$D_{test}$ ($\uparrow$)} 
& \textsc{Before} & {92.59} & {92.59} & {92.59} & 92.59 & {77.10} & {77.10} & {77.10} & 77.10  \\
& \ds{\textsc{Oracle}} & 86.28 & 90.21 & 91.01 & 89.44 & 77.49 & 64.41 & 67.06 & 66.88\\ 
& \textsc{NegGrad}  & {36.56} & {15.87} & {9.28}  & 7.11  & {\textbf{74.54}} & {48.07} & {21.11} & 10.19 \\
& \textsc{Adv}  & {74.34} & {65.14} & {62.23} & 49.47 & {60.00}  & {63.17} & {57.43} & 53.89  \\
& \textsc{Adv+Imp}  & {\textbf{77.53}} & {\textbf{79.65}} & {\textbf{67.08}} & \textbf{50.82} & {60.50} & {\textbf{63.69}} & {\textbf{62.83}} & \textbf{58.44} \\ 
\bottomrule
\end{tabular}}
\vspace{-4mm}
\label{table:main_result_dataset}
\end{table*}


\begin{table*}[!tp]
\caption{Results analogous to Table~\ref{table:main_result_dataset}, but with unlearning via relabeling each image in $\mathcal{D}_f$ to an arbitrarily chosen class. We see a similar trend where \textsc{Correct} loses significant information on $\mathcal{D}_r$, while our proposed methods retain predictive performance on $\mathcal{D}_r$ as well as $\mathcal{D}_{test}$.}
\vspace{-.1in}  
\centering
\smallskip\noindent
\resizebox{.95\linewidth}{!}{
\begin{tabular}{ll|cccc|cccc|cccc}
\toprule
&  & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{CIFAR-100} & \multicolumn{4}{c}{ImageNet-1K}\\ 
&  & {$k=4$} & {$k=16$} & {$k=64$} & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}   & $k=128$  & {$k=4$} & {$k=16$}   & {$k=64$}  & {$k=128$}    \\ \midrule
\multirow{4}{*}{$D_f$ ($\uparrow$)} 

& \textsc{Before} & {0.0} & {0.0} & {0.0} & 0.0 & {0.0} & {0.0} & {0.0} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\
& \textsc{Oracle} & 100.0 & 100.0 & 100.0 & 100.0 & 100.0  & 100.0 & 100.0 & 100.0 & & & &  \\
& \textsc{Correct}  & 100.0   & 100.0   & 100.0   & 100.0   & 100.0   & 100.0   & 100.0   & 99.84   & 100.0 & 100.0 & 100.0 & 100.0  \\
& \textsc{Adv}  & 95.0   & 100.0   & 99.375   & 98.28   & 90.0   & 100.0   & 100.0   & 98.28   & 100.0 & 100.0 & 87.5 & 71.32  \\
& \textsc{Adv+Imp}  & 90.0   & 100.0   & 53.75   & 50.16   & 80.0   & 86.25   & 20.63   & 15.16   & 100.0 & 100.0 & 8.59 & 4.30  \\
\midrule
\multirow{4}{*}{$D_r$ ($\uparrow$)}   

& \textsc{Before} & {99.60} & {99.60} & {99.60} & 99.60 & {99.98} & {99.98} & {99.98} & 99.98 & 87.42 & 87.42 & 87.42 & 87.42  \\
& \textsc{Oracle} & 94.90 & 99.73 & 99.94 & 99.90 & 97.94 & 99.90 & 99.97 & 99.79 &&& &  \\
& \textsc{Correct}  & {28.39} & {11.75} & {12.33}  & 9.71  & {\textbf{96.14}} & {74.84} & {31.79} & 18.64 & \textbf{84.34} & 82.94 & 76.21 & 68.03 \\
& \textsc{Adv}  & {81.43} & {85.53} & {83.36} & 81.06 & {69.55} & \textbf{92.94} & {94.64} & 96.32 & 70.05 & 83.09 & \textbf{84.75} &\textbf{84.54} \\
& \textsc{Adv+Imp}  & {\textbf{83.43}} & {\textbf{91.15}} & {\textbf{94.76}} & \textbf{90.57} & {68.77} & 90.73 & {\textbf{96.68}} & \textbf{96.44} & 74.18 & \textbf{83.34} & {83.27}& 80.15  \\
\midrule
\multirow{4}{*}{$D_{test}$ ($\uparrow$)} 

& \textsc{Before} & {92.59} & {92.59} & {92.59} & 92.59 & {77.10} & {77.10} & {77.10} & 77.10 & 76.01 & 76.01 & 76.01 & 76.01  \\
& \textsc{Oracle} & 87.33 & 91.65 & 91.99 & 91.57 & 71.56 & 74.05 & 74.93 & 74.15 &&& &  \\
& \textsc{Correct}  & {27.62} & {11.79} & {12.16}  & 9.80  & {\textbf{69.82}} & {53.11} & {24.37} & 14.64 & \textbf{73.26} & 71.90 & 65.68 & 58.25  \\
& \textsc{Adv}  & {76.35} & {79.15} & {76.95} & 74.61 & {51.23}  & \textbf{65.62} & {66.79} & 68.56 & 64.81 & 72.02 & \textbf{73.41} & \textbf{73.32}\\
& \textsc{Adv+Imp}  & {\textbf{78.08}} & {\textbf{84.24}} & {\textbf{86.92}} & \textbf{82.82} & {50.60} & 64.28 & {\textbf{69.15}} & \textbf{68.60} & 64.94 & \textbf{72.20} & {71.82}& {68.92} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\label{table:main_result_dataset_target}
\end{table*}


==> Tables_tex/other_results_table.tex <==
\begin{table*}[h]
    \begin{minipage}{0.48\textwidth}
        \footnotesize
         \caption{Correcting adversarial images in ImageNet-A. \textsc{Adv} achieves the least forgetting, while \textsc{Adv+Imp} fails to correct large number of predictions due to strong regularization.}
%\vspace{-0.2cm}
        \label{table:imagenet_a_results}
        \centering
        \smallskip\noindent
        \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|cccc}
            \toprule
            &  & \multicolumn{4}{c}{ImageNet-A}\\ 
            &  & {$k=16$} & {$k=32$} & {$k=64$} & $k=128$\\ 
            \midrule
            \multirow{4}{*}{$D_f$ ($\uparrow$)} 
            & \textsc{Before}  & 0.0 & 0.0 & 0.0 & 0.0 \\ 
            & \textsc{Correct}  & 100.0 & 100.0 & 100.0 & 100.0 \\ 
            & \textsc{Adv}  & 100.0 & 100.0 & 95.31 & 83.44\\ 
            & \textsc{Adv+Imp}  & 100.0 & 100.0 & 10.94 & 9.38 \\  
            \midrule
            \multirow{4}{*}{$D_r$ ($\uparrow$)}  
            & \textsc{Before}  & 87.46 & 87.46 & 87.46 & 87.46\\ 
            & \textsc{Correct}  & \textbf{84.41} & 83.29 & 80.79 & 77.38\\ 
            & \textsc{Adv}  & 81.75 & \textbf{83.80} & \textbf{83.74} & \textbf{83.44}\\ 
            & \textsc{Adv+Imp}  & 81.82 & 83.73 & 83.53 & 82.86\\ 
            \midrule
            \multirow{4}{*}{$D_{test}$ ($\uparrow$)} 
            & \textsc{Before}  & 76.15 & 76.15 & 76.15 & 76.15\\ 
            & \textsc{Correct}  & \textbf{73.21} & 72.04 & 69.91 & 66.73\\ 
            & \textsc{Adv}  & 70.89 & \textbf{72.58} & \textbf{72.68} & \textbf{72.36}\\ 
            & \textsc{Adv+Imp}  & 70.98 & 72.51 & 72.39& 71.68\\ 
            \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \footnotesize
        \caption{Unlearning instances continually by increments of $k_{CL}=8$ images per step. Our methods outperform \textsc{NegGrad} in the continual unlearning scenario as well.}
        \label{table:continual_unlearning_results}
        \centering
        \smallskip\noindent
        \resizebox{\linewidth}{!}{
        \begin{tabular}{ll|cccc}
            \toprule
            &  & \multicolumn{4}{c}{CIFAR-100 ($k_{CL}=8$)}\\ 
            &  & {$k=8$} & {$k=16$}  & {$k=64$} & {$k=128$} \\ 
            \midrule
            \multirow{4}{*}{$D_f$ ($\downarrow$)} & \textsc{Before}  & 100.0 & 100.0 & 100.0 & 100.0\\ 
            & \textsc{NegGrad}  & 0.0 & 0.0 & 0.0 & 0.52\\ 
            & \textsc{Adv}  & 0.0 & 0.0 & 1.04 & 0.0\\ 
            & \textsc{Adv+Imp}  & 0.0 & 0.0 & 0.0 & 1.04\\  
            \midrule
            \multirow{4}{*}{$D_r$ ($\uparrow$)}  & \textsc{Before}  & 99.98 & 99.98 & 99.98 & 99.98\\ 
            & \textsc{NegGrad}  & 80.58 & 31.85 & 6.60 & 1.89\\ 
            & \textsc{Adv}  & 80.33 & 70.54 & 59.67 & 38.16\\ 
            & \textsc{Adv+Imp}  & \textbf{81.46} & \textbf{72.78} & \textbf{62.30} & \textbf{47.14}\\ 
            \midrule
            \multirow{4}{*}{$D_{test}$ ($\uparrow$)} & \textsc{Before}  & 77.10 & 77.10 & 77.10 & 77.10\\ 
            & \textsc{NegGrad}  & 58.20 & 24.48 & 5.73 & 1.22\\ 
            & \textsc{Adv}  & 57.56 & 50.43 & 43.48 & 30.10\\ 
            & \textsc{Adv+Imp}  & \textbf{58.33} & \textbf{51.97} & \textbf{45.09} & \textbf{36.17}\\ 
            \bottomrule
        \end{tabular}
        }
    \end{minipage}
\end{table*}
% \vspace{-0.3cm}


==> Tables_tex/rw_comparison.tex <==
\begin{table}[!t] % 7.7cm
\centering
%\vspace{-0.3cm}
\caption{Comparison between existing unlearning methods.}
%\vspace{-0.2cm}
\footnotesize 
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llccc}
    \toprule
    Methods & Unit & Goal & $\mathcal{D}_r$ & $\mathcal{D}_f$ & Updates \\
    % Forgetting
    \midrule
    \midrule
    \citet{fastyet} &  class & undo & \cmark	& \xmark & \xmark  \\  % Arxiv % Dr_subset
    \citet{graves2021amnesiac} & class & undo &	\xmark & \xmark& \cmark    \\  % Arxiv % single class
    \citet{zeroshot} & class & undo & \xmark	& \xmark& \xmark   \\  % Arxiv 
    \citet{recoverable}& class & undo & \xmark& \cmark & \xmark  \\  % ECCV 
    \citet{fewshot} & class & undo &	\xmark & \cmark& \xmark    \\  % Arxiv % single class
    \midrule
    \citet{eternal} & instance & undo & \cmark & \cmark& \xmark  \\  % CVPR c/c
    \citet{efficienttwo} & instance & undo & \cmark & \cmark & \xmark  \\  % CVPRW 
    \citet{hessian} & instance & undo &\cmark & \cmark& \xmark   \\ % CVPR 
    \midrule
    \textbf{Ours} & \textbf{instance} & \textbf{misclassify} & \xmark & \cmark & \xmark  \\
    \bottomrule
\end{tabular}
}
%\vspace{-0.3cm}
\label{tab:comparison}
\end{table}

==> Tables_tex/supple_table.tex <==
% \begin{table}[!t]
%          \caption{Correcting adversarial images from ImageNet-A. \textsc{Adv} achieves the least forgetting, while \textsc{Adv+Imp} fails to correct large number of predictions due to strong regularization.}
%         \label{table:imagenet_a_results}
%         \vspace{-.1in}  
%         \centering
%         \footnotesize
%         \smallskip\noindent
%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{ll|ccccccc}
%             \toprule
%             &  & \multicolumn{4}{c}{ImageNet-A}\\ 
%             &  & {$k=16$} & {$k=32$} & {$k=64$} & $k=128$ & $k=256$ & $k=512$ & $k=1024$\\ 
%             \midrule
%             \multirow{4}{*}{$D_f$ ($\uparrow$)} 
%             & \textsc{Before}  & 0.0 & 0.0 & 0.0 & 0.0  & 0.20 & &\\ 
%             & \textsc{Correct}  & 100.0 & 100.0 & 100.0 & 100.0  & & &\\ 
%             & \textsc{Adv}  & 100.0 & 100.0 & 95.31 & 83.44  & 84.38 & &\\ 
%             & \textsc{Adv+Imp}  & 100.0 & 100.0 & 10.94 & 9.38  & 6.64 & &\\  
%             \midrule
%             \multirow{4}{*}{$D_r$ ($\uparrow$)}  
%             & \textsc{Before}  & 87.46 & 87.46 & 87.46 & 87.46  & & &\\ 
%             & \textsc{Correct}  & \textbf{84.41} & 83.29 & 80.79 & 77.38  & & &\\ 
%             & \textsc{Adv}  & 81.75 & \textbf{83.80} & \textbf{83.74} & \textbf{83.44} & \textbf{83.29} & &\\ 
%             & \textsc{Adv+Imp}  & 81.82 & 83.73 & 83.53 & 82.86 & 80.56 & &\\ 
%             \midrule
%             \multirow{4}{*}{$D_{test}$ ($\uparrow$)} 
%             & \textsc{Before}  & 76.15 & 76.15 & 76.15 & 76.15 & & &\\ 
%             & \textsc{Correct}  & \textbf{73.21} & 72.04 & 69.91 & 66.73 & & &\\ 
%             & \textsc{Adv}  & 70.89 & \textbf{72.58} & \textbf{72.68} & \textbf{72.36} & \textbf{72.13}& &\\ 
%             & \textsc{Adv+Imp}  & 70.98 & 72.51 & 72.39& 71.68 & 69.30 & &\\ 
%             \bottomrule
%         \end{tabular}
%         }
% \end{table}


==> Tables_tex/tab_various_model.tex <==

\begin{table*}[ht]
  \centering
\footnotesize
\begin{threeparttable}
\begin{tabular}{l|ccc|ccc|ccc}
    \toprule
    Method &
    \multicolumn{3}{c|}{MobileNetv2} &  \multicolumn{3}{c|}{SqueezeNet} &  \multicolumn{3}{c}{ViT} \\
    \midrule
     - & $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$) & $D_{te}$ ($\uparrow$) &  $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$) & $D_{te}$ ($\uparrow$) &  $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$) & $D_{te}$ ($\uparrow$) \\

    Original & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00\\
    NegGrad & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00\\
    \midrule
    Ours (Adv) & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00\\
    Ours (Adv+Imp) & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00\\
    \midrule
    
  \end{tabular}
  \caption{\ds{TODO : ?}} \label{tab:main} 
  \end{threeparttable}
\end{table*}

% \begin{table*}[ht]
%   \centering
% \footnotesize
% \begin{threeparttable}
% \begin{tabular}{l|cc|cc|cc|cc|cc}
%     \toprule
%     Methods &
%     \multicolumn{2}{c|}{ResNet34} & \multicolumn{2}{c|}{ResNext50} &  \multicolumn{2}{c|}{MobileNetv2} &  \multicolumn{2}{c|}{SqueezeNet} &  \multicolumn{2}{c}{ViT} \\
%     \midrule
%      & $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$) & $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$) & $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$)  & $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$) & $D_r$ ($\uparrow$) & $D_f$ ($\downarrow$) \\

%     Original & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
%     % Oracle & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
%     NegGrad & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
%     \midrule
%     Ours & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
%     Ours$^\ast$ & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
%     \midrule
    
%   \end{tabular}
%   \caption{TODO} \label{tab:main} 
%   \end{threeparttable}
% \end{table*}

% \begin{table*}[ht]
%   \centering
% %   \small
% \begin{threeparttable}
% \begin{tabular}{cl|cccc}
%     \toprule
%     \multirow{2}*{Model} & \multirow{2}{*}{Dataset} & \multirow{2}*{Oracle} & \multirow{2}{*}{NegGrad} & \multicolumn{2}{c}{Ours} \\
%     & & & & Adv. & Adv.+ Imp \\
%     %  Model & Dataset & Original & Oracle & NegGrad & Ours & \multicolumn{1}{c}{CHAM.} \\
%     \midrule

%     \multirow{3}{*}{MobilenetV2}
%     & $D_r$  & 00.00 & 00.00 & 00.00 & 00.00 \\
%     & $D_f$ & & & & \\
%     \cmidrule{2-6}
%     & $D_{te}$ & & & & \\
%     \midrule
    
%     \multirow{3}{*}{SqueezeNet}
%     & $D_r$   & & & & \\
%     & $D_f$ & & & & \\
%     \cmidrule{2-6}
%     & $D_{te}$ & & & & \\
%     \midrule

%     \multirow{3}{*}{ViT}
%     & $D_r$   & & & & \\
%     & $D_f$ & & & & \\
%     \cmidrule{2-6}
%     & $D_{te}$ & & & & \\

%   \end{tabular}

%   \caption{} \label{tab:main}
%   \end{threeparttable}
% \end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

